Efficient Two-Step Adversarial Defense for Deep Neural Networks

In recent years, deep neural networks have demonstrated outstanding performance in many machine learning tasks. However, researchers have discovered that these state-of-the-art models are vulnerable to adversarial examples: legitimate examples added by small perturbations which are unnoticeable to human eyes. Adversarial training, which augments the training data with adversarial examples during the training process, is a well known defense to improve the robustness of the model against adversarial attacks. However, this robustness is only effective to the same attack method used for adversarial training. Madry et al.(2017) suggest that effectiveness of iterative multi-step adversarial attacks and particularly that projected gradient descent (PGD) may be considered the universal first order adversary and applying the adversarial training with PGD implies resistance against many other first order attacks. However, the computational cost of the adversarial training with PGD and other multi-step adversarial examples is much higher than that of the adversarial training with other simpler attack techniques. In this paper, we show how strong adversarial examples can be generated only at a cost similar to that of two runs of the fast gradient sign method (FGSM), allowing defense against adversarial attacks with a robustness level comparable to that of the adversarial training with multi-step adversarial examples. We empirically demonstrate the effectiveness of the proposed two-step defense approach against different attack methods and its improvements over existing defense strategies.

==> tables/black-box-mnist.tex <==
% Table generated by Excel2LaTeX from sheet 'black-box-mnist'
\begin{table}[htbp]
  \centering
  \caption{MNIST: Performance of different models under black-box adversarial attacks. The sbustitued model are choosen from already well-trained models. The training process contains 30,000 iterations of 256 images in each iteration. ``H'' stands for defence model trained with one-hot label and ``S'' means label smoothing is using on the defence model.}
    \begin{tabular}{c||c|c|c|c|c|c|c}
    \multicolumn{1}{c}{\multirow{2}[3]{*}{Substitude Model}} & \multicolumn{1}{c}{\multirow{2}[3]{*}{Label}} & \multicolumn{1}{c}{\multirow{2}[3]{*}{Natural}} & \multicolumn{3}{c}{FGSM} & \multicolumn{1}{c}{PGD} & \multirow{2}[3]{*}{Our Method} \\
\cmidrule{4-6}    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & $\varepsilon = 0.2$ & $\varepsilon= 0.3$ & \multicolumn{1}{c}{$\varepsilon = 0.4$} & \multicolumn{1}{c}{$\varepsilon = 0.3, k = 30$} &  \\
    \midrule
    \multirow{2}[2]{*}{Natural Model} & H     & 0     & 0.8106 & 0.9412 & 0.9243 & 0.974 & \multirow{2}[2]{*}{0.9206} \\
          & S     & 0.2062 & 0.6568 & 0.8179 & 0.898 & 0.9718 &  \\
    \midrule
    \multirow{2}[2]{*}{FGSM $\varepsilon=0.3$} & H     & 0.9006 & 0.9057 & 0.082 & 0.8945 & 0.967 & \multirow{2}[2]{*}{0.9422} \\
          & S     & 0.9083 & 0.7119 & 0.7581 & 0.8215 & 0.9671 &  \\
    \midrule
    \multirow{2}[1]{*}{PGD $\varepsilon=0.3, k=30$} & H     & 0.9236 & 0.9282 & 0.9315 & 0.9145 & 0.9325 & \multirow{2}[1]{*}{0.8878} \\
          & S     & 0.8857 & 0.8657 & 0.7668 & 0.8484 & 0.9574 &  \\
    \end{tabular}%
  

  \label{table: black-box-mnist}

\end{table}%


==> tables/cifar10_configuration.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        Layer Type & Details \\ \hline
        ReLU Convolutional & 32 filters (3*3, stride 1, padding 0) \\ \hline
        ReLU Convolutional & 64 filters (3*3, stride 1, padding 0) \\ \hline
        Max Pooling & 2*2 \\ \hline
        Dropout & dropout rate:0.25 \\ \hline
        ReLU Convolutional & 128 filters (3*3, stride 1, padding 0) \\ \hline
        Max Pooling & 2*2 \\ \hline
        ReLU Convolutional & 128 filters (2*2, stride 1, padding 0) \\ \hline
        Max Pooling & 2*2, padding 1 \\ \hline
        Dropout & dropout rate:0.25 \\ \hline
        ReLU Fully Connect & 1000 units \\ \hline
        Dropout & dropout rate:0.5 \\ \hline
        Fully Connect & 10 units \\ \hline
        Softmax & 10 units \\
        \hline
    \end{tabular}
    \caption{Model configuration for CIFAR-10 data set.}
    \label{tab:cifar10-config}
\end{table}

==> tables/white-box-cifar10-test.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c||c|c|c c c|}
        \hline
         \multirow{2}{*}{Defense \textbackslash Attack} & \multirow{2}{*}{No attack} & \multirow{2}{*}{FGSM ($\varepsilon=0.06$)} & \multicolumn{3}{c|}{IFGSM ($\varepsilon=0.06$)} \\ \cline{4-6} & & & k=10 & k=20 & k=30  \\ \hline
         e2SAD & 0.73 & 0.39 & 0.333 & 0.330 & 0.328 \\ \hline
         Adv train & 0.73 & 0.41 & 0.346 & 0.343 & 0.34 \\ 
         \hline
    \end{tabular}
    \caption{Test accuracy rates of classifier trained with e2SAD and classifier trained with FGSM-based adversarial training under different attack methods.}
    \label{tab:white-box-cifar10-test}
\end{table}

==> tables/white-box-cifar10-train.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{|c||c|c|c c c|}
        \hline
         \multirow{2}{*}{Defense \textbackslash Attack} & \multirow{2}{*}{No attack} & \multirow{2}{*}{FGSM ($\varepsilon=0.06$)} & \multicolumn{3}{c|}{IFGSM ($\varepsilon=0.06$)} \\ \cline{4-6} & & & k=10 & k=20 & k=30  \\ \hline
         e2SAD & 0.94 & 0.704 & 0.627 & 0.623 & 0.620 \\ \hline
         Adv train & 0.90 & 0.635 & 0.552 & 0.548 & 0.544 \\ 
         \hline
    \end{tabular}
    \caption{Train accuracy rates of classifier trained with e2SAD and classifier trained with FGSM-based adversarial training under different attack methods.}
    \label{tab:white-box-cifar10-train}
\end{table}


==> tables/white-box-mnist.tex <==
% Table generated by Excel2LaTeX from sheet 'white-box-mnist'
\begin{table}[htbp]
  \centering  
  \caption{MNIST: Performance of different models under adversarial attacks. All compared models are trained using one-hot label and smoothing label respectively within totally 30,000 iterations of 256 images in each iteration. ``H'' stands for defence model trained with one-hot label and ``S'' means label smoothing is using on the defence model.}
    \begin{tabular}{c||c|c|c|ccc|c|c}
    \multicolumn{1}{c}{\multirow{2}[3]{*}{Attack}} & \multicolumn{1}{r}{} & \multicolumn{1}{c}{\multirow{2}[3]{*}{Label}} & \multicolumn{1}{c}{\multirow{2}[3]{*}{Natural}} & \multicolumn{3}{c}{FGSM} & \multicolumn{1}{c}{PGD} & \multirow{2}[3]{*}{Our Method} \\
\cmidrule{5-7}    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{$\varepsilon = 0.2$} & \multicolumn{1}{c|}{$\varepsilon= 0.3$} & \multicolumn{1}{c}{$\varepsilon = 0.4$} & \multicolumn{1}{c}{$\varepsilon = 0.3, k = 30$} &  \\
    \midrule
    \multirow{2}[2]{*}{Natural} & \multirow{2}[2]{*}{} & H     & 0.9942 & 0.9927 & 0.9938 & 0.9921 & 0.9913 & \multirow{2}[2]{*}{0.9932} \\
          &       & S     & 0.9952 & 0.9946 & 0.9943 & 0.9941 & 0.9913 &  \\
    \midrule
    \multirow{6}[6]{*}{FGSM} & \multirow{2}[2]{*}{$\varepsilon = 0.2$} & H     & 0.4427 & 0.9886 & 0.9714 & 0.9494 & 0.9695 & \multirow{2}[2]{*}{0.9749} \\
          &       & S     & 0.7283 & 0.9829 & 0.9824 & 0.9846 & 0.9736 &  \\
\cmidrule{2-9}          & \multirow{2}[2]{*}{$\varepsilon = 0.3$} & H     & 0.1741 & 0.9628 & 0.9768 & 0.9658 & 0.9519 & \multirow{2}[2]{*}{0.9641} \\
          &       & S     & 0.4256 & 0.9705 & 0.9846 & 0.9919 & 0.9595 &  \\
\cmidrule{2-9}          & \multirow{2}[2]{*}{$\varepsilon = 0.4$} & H     & 0.1027 & 0.7501 & 0.9136 & 0.9732 & 0.8152 & \multirow{2}[2]{*}{0.9499} \\
          &       & S     & 0.2146 & 0.9334 & 0.9374 & 0.9914 & 0.9012 &  \\
    \midrule
    \multicolumn{1}{c||}{\multirow{6}[5]{*}{PGD}} & \multirow{2}[2]{*}{k=10} & H     & 0.0001 & 0.0584 & 0.0856 & 0.2108 & 0.9336 & \multirow{2}[2]{*}{0.8687} \\
          &       & S     & 0.1019 & 0.0648 & 0.1166 & 0.0101 & 0.9422 &  \\
\cmidrule{2-9}          & \multirow{2}[2]{*}{k=15} & H     & 0.0001 & 0.0539 & 0.0817 & 0.2032 & 0.9325 & \multirow{2}[2]{*}{0.8619} \\
          &       & S     & 0.0992 & 0.0576 & 0.1037 & 0.0089 & 0.9417 &  \\
\cmidrule{2-9}          & \multirow{2}[1]{*}{k=30} & H     & 0     & 0.0575 & 0.082 & 0.1968 & 0.9325 & \multirow{2}[1]{*}{0.8633} \\
          &       & S     & 0.093 & 0.0526 & 0.0966 & 0.0065 & 0.9412 &  \\
    \end{tabular}%
  \label{table: white-box-mnist}
\end{table}%

